JWST reveals a population of ultra-red, flattened disk galaxies at 2<z<6 previously missed by HST

With just a month of data, JWST is already transforming our view of the Universe, revealing and resolving starlight in unprecedented populations of galaxies. Although ``HST-dark" galaxies have previously been detected at long wavelengths, these observations generally suffer from a lack of spatial resolution which limits our ability to characterize their sizes and morphologies. Here we report on a first view of starlight from a subset of the HST-dark population that are bright with JWST/NIRCam (4.4$\mu$m<24.5mag) and very faint or even invisible with HST ($<$1.6$\mu$m). In this Letter we focus on a dramatic and unanticipated population of physically extended galaxies ($\gtrsim$0.17''). These 12 galaxies have photometric redshifts $2<z<6$, high stellar masses $M_{\star}\gtrsim 10^{10}~M_{\odot}$, and significant dust-attenuated star formation. Surprisingly, the galaxies have elongated projected axis ratios at 4.4$\mu$m, suggesting that the population is disk-dominated or prolate. Most of the galaxies appear red at all radii, suggesting significant dust attenuation throughout. We refer to these red, disky, HST-dark galaxies as Ultra-red Flattened Objects (UFOs). With $r_e$(F444W)$\sim1-2$~kpc, the galaxies are similar in size to compact massive galaxies at $z\sim2$ and the cores of massive galaxies and S0s at $z\sim0$. The stellar masses, sizes, and morphologies of the sample suggest that some could be progenitors of lenticular or fast-rotating galaxies in the local Universe. The existence of this population suggests that our previous censuses of the universe may have missed massive, dusty edge-on disks, in addition to dust-obscured starbursts.

==> old_figure_commands.tex <==

\begin{figure*}
    \centering
    \includegraphics[trim={0 0.4cm 0 0},clip,width=\textwidth]{figures/38568_stamps.pdf}
    \includegraphics[trim={0 0.4cm 0 0.7cm},clip ,width=\textwidth]{figures/39336_stamps.pdf}
    \includegraphics[trim={0 0.4cm 0 0.7cm},clip,width=\textwidth]{figures/38029_stamps.pdf}
    \caption{2.4" x 2.4" images of three galaxies in our sample spanning 1.15-4.4\micron. We select galaxies which are bright in 4.4\micron and barely detected in 1.5\micron and 1.15\micron. The expectation was that these sources would look for the most part like the object in the first row (lil chonky bois): very compact. However, in addition to compact galaxies we find extended disks like those in the middle and bottom row (big bad disks). These remarkably red disks are very surprising.}
    \label{fig:my_label}
\end{figure*}



\begin{figure*}
\includegraphics[width=0.2\textwidth]{figures/eazyfit_35528.pdf}
\includegraphics[width=0.2\textwidth]{figures/eazyfit_30378.pdf}
\includegraphics[width=0.2\textwidth]{figures/eazyfit_30791.pdf}
\includegraphics[width=0.2\textwidth]{figures/eazyfit_38029.pdf}
\includegraphics[width=0.2\textwidth]{figures/eazyfit_26558.pdf}
\includegraphics[width=0.2\textwidth]{figures/eazyfit_33400.pdf}
\includegraphics[width=0.2\textwidth]{figures/eazyfit_39336.pdf}
\includegraphics[width=0.2\textwidth]{figures/eazyfit_35547.pdf}
\includegraphics[width=0.2\textwidth]{figures/eazyfit_38066.pdf}
\includegraphics[width=0.2\textwidth]{figures/eazyfit_38568.pdf}
\includegraphics[width=0.2\textwidth]{figures/eazyfit_9002.pdf}
\includegraphics[width=0.2\textwidth]{figures/eazyfit_37213.pdf}
\includegraphics[width=0.2\textwidth]{figures/eazyfit_36743.pdf}
\includegraphics[width=0.2\textwidth]{figures/eazyfit_375.pdf}
\includegraphics[width=0.2\textwidth]{figures/eazyfit_22739.pdf}
\includegraphics[width=0.2\textwidth]{figures/eazyfit_37054.pdf}
\includegraphics[width=0.2\textwidth]{figures/eazyfit_33642.pdf}
\includegraphics[width=0.2\textwidth]{figures/eazyfit_34424.pdf}
\includegraphics[width=0.2\textwidth]{figures/eazyfit_14924.pdf}
\end{figure*}



\begin{figure*}
    \centering
    \includegraphics[trim={0 9cm 0 0},clip,width=\textwidth]{figures/bbd_fig3.pdf}
    \caption{Color images and SEDs for four of our \redrockets. The top panels are three color images using the F150W, F277W, and F444W filters. The bottom panels show the 0.4-5\micron spectral energy distributions (SEDs) and photometric redshift probability distributions $P(z)$. These galaxies are very red and remarkably disky.}
    \label{fig:seds}
\end{figure*}

\begin{figure*}[ht!]
    \centering
    \includegraphics[width=\textwidth]{figures/selection.pdf}
    \caption{\textbf{Sample selection:} We select galaxies that are bright in F444W and are detected at $<10\sigma$ in F150W and $<10\sigma$ in F150W$<10\sigma$ in F115W. We then investigate the properties of the \redrockets\ by selecting galaxies with effective radii $r_e(F444W) > 0.2$"}
    \label{fig:selection}
\end{figure*}
%This figure shows the F160W - F444W color versus the signal-to-noise ratio in JWST F444W. 

